From Selective Deep Convolutional Features to Compact Binary Representations for Image Retrieval

In the large-scale image retrieval task, the two most important requirements are the discriminability of image representations and the efficiency in computation and storage of representations. Regarding the former requirement, Convolutional Neural Network (CNN) is proven to be a very powerful tool to extract highly discriminative local descriptors for effective image search. Additionally, in order to further improve the discriminative power of the descriptors, recent works adopt fine-tuned strategies. In this paper, taking a different approach, we propose a novel, computationally efficient, and competitive framework. Specifically, we firstly propose various strategies to compute masks, namely SIFT-mask, SUM-mask, and MAX-mask, to select a representative subset of local convolutional features and eliminate redundant features. Our in-depth analyses demonstrate that proposed masking schemes are effective to address the burstiness drawback and improve retrieval accuracy. Secondly, we propose to employ recent embedding and aggregating methods which can significantly boost the feature discriminability. Regarding the computation and storage efficiency, we include a hashing module to produce very compact binary image representations. Extensive experiments on six image retrieval benchmarks demonstrate that our proposed framework achieves the state-of-the-art retrieval performances.

==> tex/evaluation-multi-layers.tex <==
\subsubsection{Assemble features across multiple layers}
\label{sssec:multi_layer}


==> tex/evaluation-using-tine-tuned.tex <==
\subsection{Taking advantages from tine-tuned network}
Since our proposed methods take the 3D activation tensor of a convolution layer as the input, our methods are totally compatible with fine-tuned networks \cite{finetune_hard_samples,netvlad}.  In the \textbf{Fine-tuned network} section of Table \ref{tb:state-of-art}, we evaluate our best framework - $\mathcal{M}_\text{MAX} + \phi_\Delta+\psi_\text{d}$ - with the local conv. features of fine-tuned VGG for image retrieval task from \cite{netvlad,finetune_hard_samples} as input. 

Different from the results with off-the-shelf VGG network, when using local conv. features extracted from fine-tuned network from \cite{finetune_hard_samples}, our method can achieve very competitive results with those from \cite{finetune_hard_samples} at dimensionality of 512. Our method outperforms \cite{finetune_hard_samples} in majority of benchmark datasets, including {\textit{Oxford5k}}, {\textit{Oxford105k}}, {\textit{Holidays}}, and {\textit{Paris106k}}. Furthermore, at 1024 dimensionality, our method outperforms the most competitive method \cite{netvlad,finetune_hard_samples} by more than $+2.5\%$, except {\textit{Paris6k}} dataset with $+1.0\%$ performance gain to the next best \textbf{\textit{mAP}} value. It is worth to note that the end-to-end training architecture proposed in \cite{finetune_hard_samples} still inherits the drawback of upper bounded final representation dimensionality from R-MAC \cite{R-MAC}.

In Table \ref{tb:state-of-art}, ``NetVLAD fine-tuned'' represents the results reported in \cite{netvlad} after fine-tuning for differentiating the results from NetVLAD using off-the-shelf network. ``NetVLAD $\star$'' and ``siaMAC $\dagger$'' mean that the fine-tuned VGG from NetVLAD \cite{netvlad} and siaMAC \cite{finetune_hard_samples} respectively are used to extracted local conv. features as input for our proposed framework. 


% Note that we do not use re-trained model from \cite{deep_img_retr} since (i) the authors do not release the re-trained VGG model\footnote{The authors only release the re-trained ResNet \cite{resnet} model.}, and (ii) \citet{deep_img_retr} proposed to re-train the model in \textit{supervised} manner while our work mainly focus only \textit{unsupervised} aspect. We cited the results from \cite{deep_img_retr} in Table \ref{tb:state-of-art} to emphasize that our \textit{unsupervised} method can achieve a very competitive performance even with \textit{supervised} method \cite{deep_img_retr}.


% \begin{table*}[ht]
% \caption{Comparison with the state of the art.}
% \label{tb:fine-tune}
% \centering
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Dim.}} & \multicolumn{5}{c|}{\textbf{Datasets}}\\
% \cline{3-7} & & \textit{\textbf{Oxford5k}} & \textbf{\textit{Oxford105k}} & \textbf{\textit{Paris6k }}& \textbf{\textit{Paris106k}} & \textbf{\textit{Holidays}} \\
% \hline
% \hline

% % MAC fine-tuned \cite{finetune_hard_samples} & 512 & 79.7 & 73.9 &  82.4 & 74.6 & 79.5 \\
% R-MAC fine-tuned \cite{finetune_hard_samples} & 512 & 77.0 & 69.2 & 83.8 & 76.4 & 82.5 \\
% NetVLAD fine-tuned \cite{netvlad} & 1024 & 69.2 & - & 76.5 & - & 86.5 \\
% % \rowcolor{Gray}
% % Deep Image Retrieval \cite{deep_img_retr} & 512 & 83.1 & 78.6 & 87.1 & 79.7 & 89.1\\
% \hline
% R-MAC fine-tuned \cite{finetune_hard_samples} + \textbf{Our-MAX mask} & 512 & 77.7 & 72.7 & 83.2 & 76.5 & 86.3 \\
% R-MAC fine-tuned \cite{finetune_hard_samples} + \textbf{Our-MAX mask} & 1024 & 81.4 & 77.4 & 84.8 & 78.9 & 88.9 \\
% NetVLAD fine-tuned \cite{netvlad} + \textbf{Our-MAX mask} & 1024 & 75.2 & 71.7 & 84.4 & 76.9 & 91.5 \\
% \hline
% \multicolumn{7}{|c|}{\textbf{Longer dimensionality}} \\
% \hline
% NetVLAD fine-tuned \cite{netvlad} & 4096 & 71.6 & - & 79.7 & - & 87.5 \\
% NetVLAD fine-tuned \cite{netvlad} + \textbf{Our-MAX mask} & 4096 & 78.2 & 75.7 & 87.8 & 81.8 & 92.2 \\
% R-MAC fine-tuned \cite{finetune_hard_samples} + \textbf{Our-MAX mask} & 4096 & 83.8 & 80.6 & 88.3 & 83.1 & 90.1 \\

% \hline
% \end{tabular}
% \end{table*}
